A Localized-Orbital Energy Evaluation for Auxiliary-Field Quantum Monte Carlo

Phaseless Auxiliary-Field Quantum Monte Carlo (ph-AFQMC) has recently emerged as a promising method for the production of benchmark-level simulations of medium to large-sized molecules, due to its accuracy and favorable polynomial scaling with system size. Unfortunately the memory footprint of standard energy evaluation algorithms are non-trivial, which can significantly impact timings on graphical processing units (GPUs) where memory is limited. Previous attempts to reduce scaling by taking advantage of the low rank structure of the Coulombic integrals have been successful, but are significantly limited by high prefactors, rendering the utility limited to very large systems. Here, we present a complementary, cubic scaling route to reduce memory and computational scaling based on the low rank of the Coulombic interactions between localized orbitals, focusing on the application to phaseless AFQMC. We show that the error due to this approximation, which we term Localized Orbital AFQMC (LO-AFQMC), is systematic and controllable via a single variable, and is computationally favorable even for small systems. We present results demonstrating a robust retention of accuracy versus both experiment and full ph-AFQMC for a variety of test cases chosen for their potential difficulty for localized orbital based methods, including the singlet-triplet gaps of polyacenes benzene through pentacene, the heats of formation for a set of platonic hydrocarbon cages, and the total energy of ferrocene (Fe(Cp)$_2$). Finally, we reproduce our previous result of the gas phase ionization energy of Ni(Cp)$_2$, agreeing with full ph-AFQMC to within statistical error while using less than a fifteenth of the computer time.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
